On the Computational Complexity of Satisfiability Solving for String Theories

Satisfiability solvers are increasingly playing a key role in software verification, with particularly effective use in the analysis of security vulnerabilities. String processing is a key part of many software applications, such as browsers and web servers. These applications are susceptible to attacks through malicious data received over network. Automated tools for analyzing the security of such applications, thus need to reason about strings. For efficiency reasons, it is desirable to have a solver that treats strings as first-class types. In this paper, we present some theories of strings that are useful in a software security context and analyze the computational complexity of the presented theories. We use this complexity analysis to motivate a byte-blast approach which employs a Boolean encoding of the string constraints to a corresponding Boolean satisfiability problem.

==> algo.tex <==
\section{Algorithm}

Our algorithm shares a similar philosophy with the MSR
algorithm (TACAS '09): solve for a candidate length and then byte-blast.

However, the emphasis is different. We consider formulas that
mainly comprise containment and equality constraints. 

We want to minimize case-splitting by the SAT engine on possible
placements of containment. The heuristic is that mostly string
positions are fixed or only move within a small window.

Also we think it's OK to byte-blast to a larger string length
than the minimal length generated by the MSR algo -- the capacity
of SAT solvers is good enough to handle this. However, it is the
case-splitting for positioning a contained string inside a bigger
string that we need to handle.

Rough outline of the algorithm:
\begin{itemize}

\item {\em Process equalities:}
For each positive (non-negated) constraint of the form $\str = \strConst$
and $\str \strContainsAt{i} \strConst$, set the corresponding string characters
and perform constant propagation to simplify the formula.

If a contradiction is encountered during constant propagation, stop
and output UNSAT.

\item {\em Process containment constraints:}
Construct a graph where each string expression appearing in the formula
is a node and we add an edge from node $j$ to node $i$ if 
$i$ contains $j$.

Cycles in this graph indicate an equivalence class of string expressions.
These can be folded into a single node.

On the resulting DAG, perform transitive closure. Check the resulting
constraints against negated containment relations, if any exist. If a
contradiction is obtained, report UNSAT. Otherwise continue.

If a node has many child nodes, pick an ordering of the strings corresponding
to the child nodes to appear in the string corresponding to the parent node,
with filler positions in between. For each contained string, one could also 
pick a small window within which it lies (using some heuristic). 

In some sense, we are doing an under-approximation with respect to the
position of strings within a bigger string.

\item {\em Solve length constraints:} 
Create a set of length constraints similar to the
MSR work. However, the containment graph yields longer
lengths that include filler positions.

As described in the previous step, 
we also localize positions of contained strings to either fixed
positions or within small windows.

\item {\em Byte-blast with refinement:} 
If we byte-blast and get SAT, we're OK.

If we get UNSAT, then either it's really UNSAT or the ordering
of strings is wrong. The unsat core gives us an indication
of what containment orderings to reorder (similar to UCLID TACAS '07 work).

\end{itemize}

In principle, rather than iterating the abstraction-refinement
loop on candidate lengths, we're iterating it on candidate orderings
of contained strings. The idea being that such orderings are usually fixed.

NEED TO FORMALIZE THE ABOVE AND IMPLEMENT....




==> allcompl.tex <==
\section{Complexity Results}

In this section, we observe that satisfiability of any formulae in string theory as defined in Section~\ref{sec:theorydef} is in NP. This is a direct consequence of having a constant bound on the size of any string. We also prove the NP-completeness of checking the satisfiability of formulae using the following string operators with Boolean connectives. 

\begin{mylist}
\item equality and containment - EQCONT fragment of string theory
\item equality and containment at constant position - EQCAT-CONST fragment of string theory
\item equality and concatenation - EQCONC fragment of string theory
\item equality and extraction with constant indices - EQEXT-CONST fragment of string theory 
\end{mylist}

\subsection{EQCONT}

\begin{theorem}

The satisfiability problem over the theory of strings
with equality, contains, Boolean negation and conjunction (EQCONT fragment) 
is NP-hard.

\end{theorem}

\begin{proof}
We prove this by reducing 3-CNF-SAT to EQCONT fragment of theory of strings.\\
Let us consider a 3-CNF formula $\phi$ over a set $X = \{x_1,x_2,\ldots,x_n\}$
 of $n$ Boolean variables.
$$ \phi \equiv \displaystyle \bigwedge_{i=1}^m (l_1^i \vee l_2^i \vee l_3^i)$$
where each literal $l^j_i$ is $x_k$ or $\neg x_k$ for some $x_k \in X$.\\
We know that 3-CNF-SAT is NP-complete (Cook,1971).We now reduce this problem,
that is, finding an assignment of variables in
$X$ to $\{0,1\}$ such that $\phi$ evaluates to $1$, to the problem of finding
a satisfying assignment in EQCONT fragment of theory of strings.\\
\\
We describe a transformation that maps a 3-CNF Boolean formula to
a formula in EQCONT fragment of theory of strings (over the alphabet $\{a\}$) such that there is a satisfying
assignment for the Boolean formula if and only if there is a satisfying
assignment for the formula over strings.\\

Let $\psi$ be defined as 
$$ \psi(x_i) \triangleq s_i \; and \; \psi(\neg x_i) \triangleq r_i$$ 
where $s_i$ and $r_i$ are strings of atmost length $1$.
$s_i = a$ if and only if $x_i$ is assigned true, otherwise, it is $\epsilon$.
Similarly, $r_i = a$ if and only if $x_i$ is assigned false,
otherwise it is $\epsilon$.


We also need to add
constraints to ensure consistency, that is, exactly one of $x_i$ or
$\neg x_i$ is assigned true. For consistency, for each variable
$x_i$, we must have the constraint
$$s_i \not = r_i$$
This ensures that exactly one of $s_i$ or $r_i$ is $a$.

Each clause $c \equiv l_1 \vee l_2 \vee l_3$ is transformed to
$$V_c \strContains \psi(l_1)$$
$$V_c \strContains \psi(l_2)$$
$$V_c \strContains \psi(l_3)$$
$$V_c \not = \epsilon$$
where $V_c$ is a new variable for clause c and is of length atmost $3$.

Thus, atleast one of $\psi(l_i)$ must
be $a$ which is possible if and only $l_i$ is assigned true. So,
atleast one literal in each clause is true.

A set of string constraints $\psi(\phi)$ 
is obtained by applying the above transformations
to each clause $c_i$ in 3-CNF Boolean formula $\phi$ 
and taking the
There is a satisfying assignment $\mathcal I$ to $\phi$ such that
$\mathcal I(x)$ denotes the assignment to $x$, if and only, if there is an
assignment $\mathcal I'$ to $\psi(\phi)$ such that $\mathcal I'(s_i) = a$ and
$\mathcal I'(r_i) = b$ if and only if $\mathcal I(x_i) = true$.

Thus, EQCONT fragment of string theory is NP-hard.

\end{proof}

\begin{corollary}

The satisfiability problem over the theory of strings
with equality, contains at $i$ where $i$ is variable, Boolean negation and conjunction (EQCAT-VAR fragment) is NP-hard.

\end{corollary}

\begin{proof}
$str_1 \strContains str_2$ can be rewritten as $str_1 \strContainsAt i str_2$ where $i$ is a new index variable. Hence, any formula in EQCONT can be expressed
as a formula in EQCAT-VAR fragment.
\end{proof}

\subsection{EQCAT-CONST}

\begin{theorem}

The satisfiability problem over the theory of strings
with contains at constant position, equality, Boolean negation and conjunction (EQCAT-CONST fragment) 
is NP-hard.

\end{theorem}

\begin{proof}
We prove this by reducing 3-CNF-SAT to EQCAT-CONST fragment of theory of strings.\\
Let us consider a 3-CNF formula $\phi$ over a set $X = \{x_1,x_2,\ldots,x_n\}$
 of $n$ Boolean variables.
$$ \phi \equiv \displaystyle \bigwedge_{i=1}^m (l_1^i \vee l_2^i \vee l_3^i)$$
where each literal $l^j_i$ is $x_k$ or $\neg x_k$ for some $x_k \in X$.\\
We know that 3-CNF-SAT is NP-complete (Cook,1971).We now reduce this problem,
that is, finding an assignment of variables in
$X$ to $\{0,1\}$ such that $\phi$ evaluates to $1$, to the problem of finding
a satisfying assignment in EQCAT-CONST fragment of theory of strings.\\
\\
We describe a transformation that maps a 3-CNF Boolean formula to
a formula in EQCAT-CONST fragment of theory of strings (over the alphabet $\{a,b\}$) such that there is a satisfying
assignment for the Boolean formula if and only if there is a satisfying
assignment for the formula over strings.\\

Let $\psi$ be defined as 
$$ \psi(x_i) \triangleq s_i \; and \; \psi(\neg x_i) \triangleq r_i$$ 
where $s_i$ and $r_i$ are strings of atmost length $1$. To make it
exactly of length $1$, we  require
$s_i \not = \epsilon \wedge r_i \not = \epsilon$.
$s_i = a$ if and only if $x_i$ is assigned true, otherwise, it is $b$.
Similarly, $r_i = a$ if and only if $x_i$ is assigned false,
otherwise it is $b$.


We also need to add
constraints to ensure consistency, that is, exactly one of $x_i$ or
$\neg x_i$ is assigned true. For consistency, for each variable
$x_i$, we must have the constraint
$$s_i \not = r_i$$
This ensures that exactly one of $s_i$ or $r_i$ is $a$.

Each clause $c \equiv l_1 \vee l_2 \vee l_3$ is transformed to
$$V_c \strContainsAt 1 \psi(l_1)$$
$$V_c \strContainsAt 2 \psi(l_2)$$
$$V_c \strContainsAt 3 \psi(l_3)$$
$$V_c \not = bbb$$
where $V_c$ is a new variable for clause c and is of length atmost $3$.

Thus, atleast one of $\psi(l_i)$ must
be of $a$ which is possible if and only $l_i$ is assigned true. So,
atleast one literal in each clause is true.

A set of string constraints $\psi(\phi)$ 
is obtained by applying the above transformations
to Boolean formula $\phi$.
There is a satisfying assignment $\mathcal I$ to $\phi$ such that
$\mathcal I(x)$ denotes the assignment to $x$, if and only, if there is an
assignment $\mathcal I'$ to $\psi(\phi)$ such that $\mathcal I'(s_i) = a$ and
$\mathcal I'(r_i) = b$ if and only if $\mathcal I(x_i) = true$.

Thus, EQCAT-CONST fragment of string theory is NP-hard.

\end{proof}


\begin{corollary}

The satisfiability problem over the theory of strings
with contains at constant position, Boolean negation and conjunction (CAT-CONST fragment TO CHECK) is NP-hard.

\end{corollary}

\begin{proof}
In the proof above, we can replace $s_i \not = r_i$ 
by $\neg(s_i \strContainsAt 1 r_i)$ and $V_c \not = bbb$ by
$\neg(V_c \strContainsAt 1 bbbb)$. The NP-hardness proof still 
goes through. Dis-equality
between the strings of same length
can be expressed as dis-containment-at-1.
\end{proof}

  
\subsection{EQCONC}

\begin{theorem}

The satisfiability problem over the theory of strings
with equality, concat and Boolean conjunction (EQCONC fragment) is NP-hard.

\end{theorem} 


\begin{proof}
We prove this by reducing 3-CNF-SAT to EQCONC fragment of theory of strings.\\
Let us consider a 3-CNF formula $\phi$ over a set $X = \{x_1,x_2,\ldots,x_n\}$
 of $n$ Boolean variables.
$$ \phi \equiv \displaystyle \bigwedge_{i=1}^m (l_1^i \vee l_2^i \vee l_3^i)$$
where each literal $l^j_i$ is $x_k$ or $\neg x_k$ for some $x_k \in X$.\\
We know that 3-CNF-SAT is NP-complete (Cook,1971).We now reduce this problem,
that is, finding an assignment of variables in
$X$ to $\{0,1\}$ such that $\phi$ evaluates to $1$, to the problem of finding
a satisfying assignment in EQCONC fragment of theory of strings.\\
\\
We describe a transformation that maps a 3-CNF Boolean formula to
a formula in EQCONC fragment of theory of strings (over the alphabet $\{a\}$) such that there is a satisfying
assignment for the Boolean formula if and only if there is a satisfying
assignment for the formula over strings.\\
Let $\psi$ be defined as 
$$ \psi(x_i) \triangleq s_i \; and \; \psi(\neg x_i) \triangleq r_i$$ 
where $s_i$ and $r_i$ are strings of atmost length $1$.
$s_i = a$ if and only if $x_i$ is assigned true, otherwise, it is $\epsilon$.
Similarly, $r_i = a$ if and only if $x_i$ is assigned false,
otherwise it is $\epsilon$. So, for any literal $l$, $\psi(l)$ would be
$a$ if and only if $l$ is assigned true. We also need to add
constraints to ensure consistency, that is, exactly one of $x_i$ or
$\neg x_i$ is assigned true. For consistency, for each variable
$x_i$, we must have the constraint
$$s_i \concat r_i = a$$
This ensures that exactly one of $s_i$ or $r_i$ is $a$, that is,
exactly one of $\psi(x_i)$ or $\psi(\neg x_i)$ is $a$.

Each clause $l_1 \vee l_2 \vee l_3$ is transformed to
$$\psi(l_1) \concat \psi(l_2) \concat \psi(l_3)   \concat p_i =
aaa$$ 
where $p_i$ is of length atmost $2$.
Thus, the sum of the lengths of $\psi(l_1)$, $\psi(l_2)$ and
$\psi(l_3)$ must be atleast 1, that is, atleast one of $\psi(l_i)$ must
be $a$ which is possible if and only $l_i$ is assigned true. So,
atleast one literal in each clause is true.

A set of string constraints $\psi(\phi)$ 
is obtained by applying the above transformations
to Boolean formula $\phi$.
There is a satisfying assignment $\mathcal I$ to $\phi$ such that
$\mathcal I(x)$ denotes the assignment to $x$, if and only, if there is an
assignment $\mathcal I'$ to $\psi(\phi)$ such that $\mathcal I'(s_i) = a$ and
$\mathcal I'(r_i) = \epsilon$ if and only if $\mathcal I(x_i) = true$.

Thus, EQCONC fragment of string theory is NP-hard.

\end{proof}

Note that as a corollary of the above theorem, we obtain the following
result.

\begin{corollary}

The satisfiability problem over the theory of strings with equality and
concat (without Boolean conjunction) is NP-hard.

\end{corollary}

\begin{proof}

Introduce a new letter in the alphabet and use concat with 
the new letter $b$ as separators to replace conjunctions. 
$str_1 = str_2 \wedge str_3 = str_4$ can be replaced by a single constraint 
$str_1 \concat b \concat str_3 = str_2 \concat b \concat str_4$ where $b$ 
is a new letter. This is possible because we do not have any negation in
this fragment.

\end{proof}


\begin{corollary}

The satisfiability problem over the theory of strings
with contains ($\strContains$) and concat (CONTCONC fragment) is NP-hard.

\end{corollary} 

\begin{proof}
Equality can be expressed with two-way containment.

\end{proof}

\subsection{EQEXT-CONST}

\begin{theorem}

The satisfiability problem over the theory of strings
with equality, extract with constant indices, Boolean negation and conjunction (EQEXT-CONST fragment) is NP-hard.

\end{theorem} 


\begin{proof}
We prove this by reducing EQCAT-CONST to EQEXT-CONST fragment of theory of strings.\\
Let us consider a 3-CNF formula $\phi$ over a set $X = \{x_1,x_2,\ldots,x_n\}$
 of $n$ Boolean variables.
$$ \phi \equiv \displaystyle \bigwedge_{i=1}^m (l_1^i \vee l_2^i \vee l_3^i)$$
where each literal $l^j_i$ is $x_k$ or $\neg x_k$ for some $x_k \in X$.\\
We know that 3-CNF-SAT is NP-complete (Cook,1971).We now reduce this problem,
that is, finding an assignment of variables in
$X$ to $\{0,1\}$ such that $\phi$ evaluates to $1$, to the problem of finding
a satisfying assignment in EQEXT-CONST fragment of theory of strings.\\
\\
We describe a transformation that maps a 3-CNF Boolean formula to
a formula in EQEXT-CONST fragment of theory of strings (over the alphabet $\{a,b\}$) such that there is a satisfying
assignment for the Boolean formula if and only if there is a satisfying
assignment for the formula over strings.\\
Let $\psi$ be defined as 
$$ \psi(x_i) \triangleq s_i \; and \; \psi(\neg x_i) \triangleq r_i$$ 
where $s_i$ and $r_i$ are strings of atmost length $1$. To make it
exactly of length $1$, we  require
$s_i \not = \epsilon \wedge r_i \not = \epsilon$.
$s_i = a$ if and only if $x_i$ is assigned true, otherwise, it is $b$.
Similarly, $r_i = a$ if and only if $x_i$ is assigned false,
otherwise it is $b$.


We also need to add
constraints to ensure consistency, that is, exactly one of $x_i$ or
$\neg x_i$ is assigned true. For consistency, for each variable
$x_i$, we must have the constraint
$$s_i \not = r_i$$
This ensures that exactly one of $s_i$ or $r_i$ is $a$.

Each clause $c \equiv l_1 \vee l_2 \vee l_3$ is transformed to
$$V_c[1:1] = \psi(l_1)$$
$$V_c[2:2] = \psi(l_2)$$
$$V_c[3:3] = \psi(l_3)$$
$$V_c \not = bbb$$
where $V_c$ is a new variable for clause c and is of length atmost $3$.

Thus, atleast one of $\psi(l_i)$ must
be of $a$ which is possible if and only $l_i$ is assigned true. So,
atleast one literal in each clause is true.

A set of string constraints $\psi(\phi)$ 
is obtained by applying the above transformations
to Boolean formula $\phi$.
There is a satisfying assignment $\mathcal I$ to $\phi$ such that
$\mathcal I(x)$ denotes the assignment to $x$, if and only, if there is an
assignment $\mathcal I'$ to $\psi(\phi)$ such that $\mathcal I'(s_i) = a$ and
$\mathcal I'(r_i) = \epsilon$ if and only if $\mathcal I(x_i) = true$.

Thus, EQEXT-CONST fragment of string theory is NP-hard.

\end{proof}

\subsection{Implication to Satisfiability Solving}
Enumerate

\subsection{Conclusion}
Justification for bit-blasting to SAT

\newpage


==> disc.tex <==
\section{Discussion}

Discuss how different string solvers work - length abstraction, bitblast: how
does complexity result relate to these approaches.

Under-approximating the position at which sub-strings might appear in a string.
TACAS paper like approach. Elaborate.

